Scalable and Resource-Efficient Second-Order Federated Learning via Over-the-Air Aggregation

Second-order federated learning (FL) algorithms offer faster convergence than their first-order counterparts by leveraging curvature information. However, they are hindered by high computational and storage costs, particularly for large-scale models. Furthermore, the communication overhead associated with large models and digital transmission exacerbates these challenges, causing communication bottlenecks. In this work, we propose a scalable second-order FL algorithm using a sparse Hessian estimate and leveraging over-the-air aggregation, making it feasible for larger models. Our simulation results demonstrate more than $67\%$ of communication resources and energy savings compared to other first and second-order baselines.

==> conclustion.tex <==
\section{Conclusion}
In this letter, we introduced OTA Fed-Sophia, a scalable second-order method for FL that leverages curvature information through a sparse estimate of the Hessian matrix, rendering it suitable for larger models. Furthermore, OTA Fed-Sophia shows substantial improvements through the utilization of OTA aggregation. Our numerical results highlight OTA Fed-Sophia's superior convergence speed and enhanced bandwidth utilization compared to state-of-the-art baselines. %Future work will investigate the convergence analysis of OTA Fed-Sophia and evaluate its performance in non-IID data distributions.


